The Candidate Progenitor Companion Star of the Type Ib/c SN 2013ge

This Letter presents the detection of a source at the position of the Type Ib/c supernova (SN) 2013ge more than four years after the radioactive component is expected to have faded. This source could mark the first post-SN direct detection of a surviving companion to a stripped-envelope Type Ib/c explosion. We test this hypothesis and find the shape of the source's spectral energy distribution is most consistent with that of a B5 I supergiant. While binary models tend to predict OB-type stars for stripped-envelope companions, the location of the source on a color-magnitude diagram (CMD) places it redward of its more likely position on the main sequence (MS). The source may be temporarily out of thermal equilibrium, or a cool and inflated non-MS companion, which is similar to the suggested companion of Type Ib SN 2019yvr that was constrained from pre-SN imaging. We also consider other possible physical scenarios for the source, including a fading SN, circumstellar shock interaction, line of site coincidence, and an unresolved host star cluster, all of which will require future observations to more definitively rule out. Ultimately, the fraction of surviving companions ("binary fraction") will provide necessary constraints on binary evolution models and the underlying physics.

==> tab_hst_deluxe.tex <==
%\begin{tabular}{lccccr}\label{table:SN_comp}
\begin{deluxetable*}{ l l l l ll l}
\caption{{\it HST}/WFC3 Imaging \label{tab:tab1}}
\tablehead{
\colhead{UT Date} & \colhead{MJD} & \colhead{Epoch} & \colhead{Filter} & \colhead{Exposure} & \colhead{SN Magnitude} & \colhead{Star B Magnitude}\\
\colhead{}     & \colhead{} & \colhead{(days)} &    \colhead{}   & \colhead{(s)}      & \colhead{Vega (err)} & \colhead{Vega (err)}
    }
\startdata
\hline
\multirow{2}{*}{20161031} & \multirow{2}{*}{57692} & \multirow{2}{*}{1088} & F814W & 780 & 23.84 (0.09) & 25.67 (0.25)\\
    &   &   & F555W & 710 & 24.41 (0.05)  & 25.54 (0.08)\\
\hline
\multirow{2}{*}{20170601} & \multirow{2}{*}{57905} & \multirow{2}{*}{1301} & F300X & 1200 & ---  & ---\\
    &   &   & F475X & 350 & ---  & ---\\
\hline
\multirow{2}{*}{20190502} & \multirow{2}{*}{58605} & \multirow{2}{*}{2001} & F814W & 780 & 24.79 (0.14)  & 25.77 (0.30)\\
    &   &   & F555W & 710 & 25.36 (0.11)  & 25.44 (0.12)\\
\hline
\multirow{4}{*}{20201026} & \multirow{4}{*}{59148} & \multirow{4}{*}{2544} & F275W & 13803 & 25.03 (0.13)  & 25.04 (0.09)\\
    &   &   & F336W & 8090 &  24.96 (0.05)  & 24.75 (0.05)\\
    &   &   & F438W & 1000 & 25.83 (0.15)  & 25.87 (0.17)\\
    &   &   & F555W & 700 & 26.23 (0.17)  & 25.57 (0.11)\\
\hline
\enddata
\end{deluxetable*}

